Qubit Mapping and Routing via MaxSAT

Near-term quantum computers will operate in a noisy environment, without error correction. A critical problem for near-term quantum computing is laying out a logical circuit onto a physical device with limited connectivity between qubits. This is known as the qubit mapping and routing (QMR) problem, an intractable combinatorial problem. It is important to solve QMR as optimally as possible to reduce the amount of added noise, which may render a quantum computation useless. In this paper, we present a novel approach for optimally solving the QMR problem via a reduction to maximum satisfiability (MAXSAT). Additionally, we present two novel relaxation ideas that shrink the size of the MAXSAT constraints by exploiting the structure of a quantum circuit. Our thorough empirical evaluation demonstrates (1) the scalability of our approach compared to state-of-the-art optimal QMR techniques (solves more than 3x benchmarks with 40x speedup), (2) the significant cost reduction compared to state-of-the-art heuristic approaches (an average of ~5x swap reduction), and (3) the power of our proposed constraint relaxations.

==> 10Artifact.tex <==
% LaTeX template for Artifact Evaluation V20201122
%
% Prepared by 
% * Grigori Fursin (cTuning foundation, France) 2014-2020
% * Bruce Childers (University of Pittsburgh, USA) 2014
%
% See examples of this Artifact Appendix in
%  * SC'17 paper: https://dl.acm.org/citation.cfm?id=3126948
%  * CGO'17 paper: https://www.cl.cam.ac.uk/~sa614/papers/Software-Prefetching-CGO2017.pdf
%  * ACM ReQuEST-ASPLOS'18 paper: https://dl.acm.org/citation.cfm?doid=3229762.3229763
%
% (C)opyright 2014-2020
%
% CC BY 4.0 license
%

\special{papersize=8.5in,11in}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% When adding this appendix to your paper, 
% please remove above part
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendix
\section{Artifact Appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

This software artifact includes the source code for \ours (our MaxSAT-based tool for solving the qubit mapping and routing problem), the benchmark suite used in our evaluation, 
and scripts for invoking \ours and baseline tools on those benchmarks while collecting relevant statistics.

\subsection{Artifact check-list (meta-information)}



{\small
\begin{itemize}
  \item {\bf Algorithm: MaxSAT-based solver for qubit mapping and routing problem}
  \item {\bf Program: \ours }
  \item {\bf Compilation: gcc 9.4.0,  Python 3.8 }
  \item {\bf Data set: 160 .qasm files included in artifact }
  \item {\bf Run-time environment: Docker container running Ubuntu 20.04 (similar Linux environments should also work) }

  \item {\bf Metrics: Execution time and gates added }
  \item {\bf Output: QASM files for mapped circuits, summary statistics, plots }
  \item {\bf Experiments: Application of \ours and baseline tools on a set of 160 benchmark quantum circuits}
  \item {\bf How much disk space required (approximately)?: 10GB  }
  \item {\bf How much time is needed to prepare workflow (approximately)?: 30 minutes}
  \item {\bf How much time is needed to complete experiments (approximately)?: About 500 CPU-hours to execute full experiments }
  \item {\bf Publicly available?: Yes}
  \item {\bf Code licenses (if publicly available)?: Apache 2.0}

  \item {\bf Archived (provide DOI)?: Yes, 10.5281/zenodo.6974632}
\end{itemize}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{How to access}
Our artifact is available via GitHub (\url{https://github.com/qqq-wisc/satmap/}) and archived (\url{https://doi.org/10.5281/zenodo.6974632}).
 \subsubsection{Hardware dependencies}\
An x86-64 architecture is recommended for \verb+docker+ virtualization. 
\subsubsection{Software dependencies}
\begin{itemize}
\item GMP (included in \verb|docker| image)
\item Open-WBO-Inc (included in artifact)
\item Python 3.8 with various packages (included in \verb|docker| image)

\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}
\begin{enumerate}
\item \textbf{Setup the runtime environment} 

Install \verb+docker+ (\url{https://docs.docker.com/get-docker/}) and then pull the \verb+docker+ image with the command:
 

\verb+docker pull abtinm/qmapping:artifact+
\item \textbf{Acquire the software artifact} 

To obtain the source code for \ours and the OpenWBO-Inc MaxSAT solver, either clone the \verb+git+ repository with the \verb+--recurse-submodules+ flag or download and unzip the archive.
\item \textbf{Start container and mount the artifact}

From the \verb+satmap/+ directory, mount the artifact in the Docker container as a volume with the command:

\verb+docker run -itv "$(pwd):/home/" abtinm/qmapping+ 

\item \textbf{Build the MaxSAT solver}

\begin{verbatim}
cd home/lib/Open-WBO-Inc/
make r
\end{verbatim}

\item \textbf{Test the installation}

Return to the \verb+home/+ directory and provide execution permissions to the bash scripts with:

\verb|chmod +x *.sh|

Use the script \verb+./functional.sh+ to test the installation. 
If everything is working, the script should run \ours on a few small benchmarks and save the output in the \verb+results/+ directory.

\end{enumerate} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}

In order to precisely recreate the experimental conditions of \cref{fig:barchart_jku} and \cref{fig:barchart_all}, simply run the script \verb+fig_10_11.sh+. Similarly, to recreate \cref{fig:heuristic}, run the script \verb+fig_12.sh+. 
The \verb+results/+ folder is populated with \verb+.qasm+ files representing the output circuit and \verb+.txt+ files with summary statistics. However, the full experiments are estimated to require about 500 CPU-hours. Therefore, we also include smaller-scale versions of each of these with fewer benchmarks and configurations that execute in about 10 CPU-hours each. 
These are called \verb+fig_10_11_limited.sh+ and \verb+fig_12_limited.sh+ respectively.

All four scripts generate plots as they run with the data collected thus far. These can be found in the \verb+plots/+ directory.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected results}

Executing the full \verb+fig_10_11.sh+ and \verb+fig_12.sh+ will reproduce the corresponding figures in the paper. The limited versions of these scripts will generate similar plots that support the same qualitative claims of (1) significant scalability improvements relative to state-of-the-art constraint-based techniques and (2) significant cost reduction compared to state-of-the-art heuristic approaches.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment customization}
The \verb+experiment_runner.py+ script takes command line arguments specifying a \emph{run}: the application of a solver to a benchmark, potentially with various optional configurations. Some of these are solver-specific: such as the slice size used by \ours and the optimization objective used by \olsq. Others can be meaningfully applied to any solver such as the target connectivity graph or timeout. 

For convenience, we have provided the script \verb+run_from_arg_file.sh+ for automatically executing batches of runs. It expects the path to a file specifying a set of runs such that the arguments for each run are on a new line. To run a custom experiment, simply generate a file in the appropriate format and pass it to \verb+run_from_arg_file.sh+. See \verb+fig_10_11.sh+ and \verb+fig_12.sh+ for examples of this workflow.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Notes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% When adding this appendix to your paper, 
% please remove below part
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


